Tick-Tock on the Open Fronthaul: Securing Synchronization in O-RAN

The Precision Time Protocol (PTP) provides the time and phase synchronization required by disaggregated Open Radio Access Networks (O-RAN). Yet, in current open fronthaul deployments, PTP traffic lacks mandatory authentication and integrity protection, leaving synchronization vulnerable to spoofing, replay, and delay manipulation attacks that can degrade radio access performance. Existing protections are poorly suited to this setting: they either add excessive latency, do not support multicast dissemination efficiently, or fail to contain key exposure under partially trusted RUs. This paper analyzes the security risks of unprotected O-RAN PTP and develops a threat model for open fronthaul deployments. We then introduce PRTESLA-C, a lightweight synchronization protection mechanism that combines per-round delayed key disclosure with ASCON-based message authentication. PRTESLA-C uses an apply-then-verify-and-correct paradigm: timing samples are applied immediately to preserve real-time control, verified after key disclosure, and removed from persistent synchronization state if authentication fails. This design maintains sub-microsecond synchronization accuracy, provides strong protection against spoofing and replay, and bounds the impact of delay manipulation with minimal computational and latency overhead.

==> algos/overview_algo.tex <==

\begin{algorithm*}[t]
\caption{\sys Protocol Flow}
\label{alg:unified-ptp-tesla-ascon}
\small
\raggedright
\textbf{Input/Params:} disclosure delay $d$ (rounds, equals \texttt{DELAY}); round interval $T_{\text{int}}$ (\texttt{Tint});
anchor time $T_0$ (\texttt{Ti}); per-epoch chain length $N$ (\texttt{KN});
epoch preannounce margin $R$ (\texttt{R}); 
% seq replay window $W$ (\texttt{seqid\_window});
bounded correction/slew $S_{\max}$ (optional, for apply-then-verify-and-correct). \\
\textbf{State at DU (Master):} for each RU/device $\mathsf{dev}$, maintain current epoch id $e$,
current round index $i$, reverse-hash key chain $\{K_i\}$ (and derived MAC keys),
and next-epoch prepared chain $\{K'_i\}$ when preannouncement starts. \\
\textbf{State at RU (Slave):} for each DU device-id $\mathsf{dev}$, maintain:
(1) message store for a \emph{unified round bundle} (Sync/Follow\_Up/Delay\_Req/Delay\_Resp) keyed by seq;
(2) stored MAC per round;
(3) TESLA key-verification state: $\texttt{prev\_key}$ and $\texttt{verified\_key\_i}$ (gap-tolerant);
(4) epoch rollover cache: $(e_{\text{cur}}, e_{\text{next}}, \texttt{switch\_seq}, \texttt{next\_commit})$.

\hrulefill
% \vspace{-1mm}
% \textbf{Protocol (event-driven by PTP messages; one logical round is identified by PTP \texttt{seq})}
% \vspace{-2mm}
\hrulefill

\begin{algorithmic}[1]
\item \textbf{(Bootstrap via ANNOUNCE)} DU periodically sends \texttt{ANNOUNCE} carrying an \texttt{AuthTLV\_Announce}:
$(d, T_{\text{int}}, T_0, e_{\text{cur}}, \texttt{prev\_key})$.
RU on first valid receipt caches $d,T_{\text{int}},T_0,e_{\text{cur}}$ and initializes $\texttt{prev\_key}$.

\item \textbf{(DU$\rightarrow$RU: Sync / Follow\_Up; no MAC TLV)} For each round \texttt{seq},
DU sends \texttt{Sync(seq)} and \texttt{Follow\_Up(seq)} as normal PTP messages \emph{without} authentication TLV.

\item \textbf{(RU: receive Sync/Follow\_Up; accumulate only)} Upon receiving \texttt{Sync} or \texttt{Follow\_Up}:
\begin{itemize}
  \item apply seq replay check (drop obvious replays);
  % /window check $W$ if enabled (drop obvious replays/out-of-window);
  \item store the \texttt{seq} and message internal buffer slot (per-device mapping);
  \item do \emph{not} verify MAC now (no TLV present).
\end{itemize}

\item \textbf{(RU$\rightarrow$DU: Delay\_Req; no MAC TLV)} RU sends \texttt{Delay\_Req(seq)} and stores it into the same per-seq bundle buffer.

\item \textbf{(DU: on Delay\_Req, finalize bundle and compute MAC in Delay\_Resp)} When DU is ready to answer round \texttt{seq}:
\begin{enumerate}
  \item DU stores the \texttt{Delay\_Resp(seq)} into the same bundle buffer (so bundle now contains Sync/Follow\_Up/Delay\_Req/Delay\_Resp messages and sequence number).
  \item DU computes current logical index $i \leftarrow f(\texttt{seq})$ (device-local), selects a MAC key derived from chain position $(i+d)$, and computes
  \[
     \texttt{MAC}_i \gets \textsf{ASCON\_MAC}(\textsf{MacKey}_{i+d},\; \textsf{BundleTS}(\texttt{seq})).
  \]
  \item DU sets \texttt{disclosed\_key} $\gets K_i$ (the TESLA key disclosed at index $i$),
  and constructs \texttt{AuthTLV\_DelayResp}:
  \[
    (\texttt{MAC}_i, K_i, e_{\text{cur}}, \texttt{seq}, \texttt{switch\_point}, \texttt{NextEpochInfo}).
  \]
\end{enumerate}

\item \textbf{(Epoch preannounce piggyback)} If remaining rounds in current epoch $\le R$, then the preannouncement starts:
DU generates next epoch chain commitment, sets \texttt{switch\_point}=1 for multiple rounds near the end, and appends \texttt{NextEpochInfo} $\leftarrow$
$(e_{\text{next}}, \texttt{switch\_seq}, \texttt{next\_commit})$ into \texttt{AuthTLV\_DelayResp}, where \texttt{next\_commit} includes initial key of next epoch.
Otherwise \texttt{switch\_point}=0 and no next-epoch info is attached.

\item \textbf{(DU$\rightarrow$RU: Delay\_Resp + AuthTLV)} DU sends \texttt{Delay\_Resp(seq)} with the above authentication TLV.

\item \textbf{(RU: receive Delay\_Resp; validate seq and timing; parse TLV and cache)} 
Upon receiving \texttt{Delay\_Resp}, RU first performs lightweight admission checks: (i) a replay check on \texttt{seq} to discard obvious replays packets; and (ii) an interval-timing check to drop responses arriving outside the acceptable one-round window.
For a valid \texttt{Delay\_Resp}, RU stores the message into the per-seq bundle buffer, then parses
\texttt{AuthTLV\_DelayResp} to extract $(\texttt{MAC}_i, K_i, e_{\text{curr}}, \texttt{switch\_point}, \texttt{NextEpochInfo})$.
If \texttt{switch\_point}=1 and NextEpochInfo present, RU caches $(e_{\text{next}}, \texttt{switch\_seq}, \texttt{next\_commit})$.

\item \textbf{(RU: epoch transition rule)} If the received epoch id $e$ indicates entering the next epoch (e.g., equals cached $e_{\text{next}}$),
RU switches epoch context, resets per-epoch index state (e.g., $i\leftarrow 0$),
and updates the verification anchor appropriately (using cached \texttt{next\_commit} and initial key as the new commitment basis).

\item \textbf{(RU: TESLA key verification, gap-tolerant)} RU verifies disclosed key $K_i$ using reverse-hash chain logic:
\[
   \textsf{Hash}^{(i-\texttt{verified\_key\_i})}(K_i) \stackrel{?}{=} \texttt{prev\_key},
\]
where \texttt{verified\_key\_i} is the last verified index (allows gaps/loss).
On success: set \texttt{prev\_key} $\leftarrow K_i$ and \texttt{verified\_key\_i}$\leftarrow i$.
On failure: mark verification failure for the corresponding stored round(s) and abort MAC verification.

\item \textbf{(RU: delayed MAC verification for round $i-d$)} If $i<d$, skip MAC verification (bootstrapping window).
Else:
\begin{enumerate}
  \item Derive MAC key from disclosed key $K_i$ using the same context derivation as DU.
  \item Locate the stored bundle for round $(i-d)$ from the per-device mapping and recompute:
  \[
     \widehat{\texttt{MAC}}_{i-d} \gets \textsf{ASCON\_MAC}(\textsf{MacKey}_{i},\; \textsf{BundleTS}(\texttt{seq}_{i-d})).
  \]
  \item Compare with stored $\texttt{MAC}_{i-d}$; record \texttt{SUCCESS/FAILED} in a per-round ledger.
\end{enumerate}

\item \textbf{Correction} RU may \emph{speculatively} apply time offset corrections once a round bundle is complete, bounded by $S_{\max}$, and later:
if the delayed verification for that round fails, RU performs decontamination/correction using the stored ledger (bounded, no hard rollback).

\item \textbf{Garbage collection and timeout check} RU periodically frees per-round bundle/MAC storage once it is verified, or if it becomes unverifiable due to missing components beyond a timeout.
\end{algorithmic}
\end{algorithm*}

% \begin{algorithm*}[t]
% \caption{Protocol Flow: \sys with Loss Resilience and Seamless Rollover}
% \label{alg:unified-prteslaC}
% \small
% \raggedright
% {\textbf{Input:} Disclosure delay $d$ (rounds); round rate $r$ ($T_{\text{round}}=1/r$); max slew $S_{\max}$;
% verification timeout $\tau_{\text{verify}}$; optional seq jump bound $W_{\text{seq}}$;
% rollover preannounce margin $R_{\text{roll}}$; window retransmission params $(w,K_{\text{win}})$.
% DU holds reverse-hash-chain keys $K_{\texttt{seq}}$ per epoch and commitments; RU knows $\texttt{Commit}_{\text{cur}}$ and maintains per-round buffers.}

% \textbf{Output:} RU maintains realtime synchronization via apply-then-verify-and-correct while tolerating loss/reordering; DU provides delayed key disclosure and seamless key rollover.

% \hrulefill \vspace{-1mm}

% \textbf{Protocol (event-driven, per round $\texttt{seq}$)} \\
% \vspace{-2mm}
% \hrulefill

% \begin{algorithmic}[1]
% \item \textbf{(DU$\rightarrow$RU: Sync/Follow\_Up)} DU sends \texttt{Sync}(\texttt{seq})/\texttt{Follow\_Up}(\texttt{seq}).
%        If available, piggyback $\texttt{PrevMAC} \gets (\texttt{seq}-1,\texttt{MAC}_{\texttt{seq}-1})$ \hfill \emph{(redundancy A)}.
% \item \textbf{(RU: seq handling)} Upon receipt, RU applies gap-tolerant seq logic:
%       if $\texttt{seq} < \texttt{expected\_seq}$ drop; if $\texttt{seq}>\texttt{expected\_seq}$ mark missing rounds and advance \texttt{expected\_seq}.
%       RU stores timestamps/messages into $\texttt{measbuf}[\texttt{seq}]$ and stores any received \texttt{PrevMAC} into $\texttt{macbuf}$.

% \item \textbf{(RU$\rightarrow$DU: Delay\_Req)} RU sends \texttt{Delay\_Req}(\texttt{seq}) and stores its local timestamps in $\texttt{measbuf}[\texttt{seq}]$.

% \item \textbf{(DU$\rightarrow$RU: Delay\_Resp + MAC)} DU derives $K_{\texttt{seq}}$ and computes
%       $\texttt{MAC}_{\texttt{seq}} \gets \texttt{MAC}(K_{\texttt{seq}}, \texttt{bundle}(\texttt{seq}) \,\|\, \texttt{seq} \,\|\, \texttt{chain\_id})$,
%       then attaches $\texttt{MAC}_{\texttt{seq}}$ to \texttt{Delay\_Resp}(\texttt{seq}) and sends it.
%       DU enqueues $(\texttt{seq},K_{\texttt{seq}},\texttt{disclose\_at}=\texttt{seq}+d)$ into \texttt{discloseQ}.

% \item \textbf{(RU: assemble \& apply)} RU stores \texttt{Delay\_Resp} timestamps into $\texttt{measbuf}[\texttt{seq}]$ and (if present) stores $\texttt{MAC}_{\texttt{seq}}$ into $\texttt{macbuf}[\texttt{seq}]$.
%       If $\texttt{RoundComplete}(\texttt{measbuf}[\texttt{seq}])$ holds, RU computes \texttt{offset} and calls \texttt{ApplySpeculativeUpdate}(\texttt{seq}, \texttt{offset}) using bounded slew ($\le S_{\max}$),
%       records $\texttt{ledger}[\texttt{seq}]$, and sets $\texttt{verify\_deadline}[\texttt{seq}] \gets \texttt{now}+\tau_{\text{verify}}$.
%       Otherwise (incomplete round, e.g., lost \texttt{Delay\_Resp}), RU skips the round and does not apply any update.

% \item \textbf{(DU$\rightarrow$RU: optional WinMAC)} If $(\texttt{seq} \bmod K_{\text{win}} = 0)$, DU sends low-rate \texttt{WinMAC} list
%       $\{(\texttt{seq}-j,\texttt{MAC}_{\texttt{seq}-j})\}_{j=1}^{w}$ in \texttt{Announce}/management \hfill \emph{(redundancy B)}.
%       RU uses it to fill missing entries in $\texttt{macbuf}[\cdot]$.

% \item \textbf{(DU$\rightarrow$RU: key disclosure)} When \texttt{discloseQ} head becomes due (at round $\texttt{seq}$), DU discloses key $K_{\texttt{seq}-d}$ along with its index.
%       RU triggers \texttt{VerifyAndPossiblyCorrect}(\texttt{seq}-d): it verifies the key against $\texttt{Commit}_{\text{cur}}$ (or previous epoch during transition), recomputes the MAC, and
%       (i) if valid, commits/cleans up; (ii) if invalid, calls \texttt{CorrectUsingLedger}(\texttt{seq}-d) (state decontamination + bounded slew, no hard rollback).

% \item \textbf{(Garbage collection)} RU periodically checks $\texttt{verify\_deadline}[\cdot]$; if expired without verification, mark \texttt{UNVERIFIABLE} and free $\texttt{measbuf}/\texttt{macbuf}/\texttt{ledger}$ for that round.

% \item \textbf{(Rollover preannounce)} If remaining rounds in the current epoch $\le R_{\text{roll}}$, DU piggybacks authenticated \texttt{NextCommit} and \texttt{switch\_seq} on regular messages for multiple rounds.
%       RU caches \texttt{Commit\_next}. At \texttt{switch\_seq}, RU activates \texttt{Commit\_next}; if missing, RU enters holdover until it is received.
% \end{algorithmic}

% \end{algorithm*}

% \setlength{\floatsep}{0.1cm}





==> tables/comparison.tex <==
\begin{table}[t]
\centering
\caption{Comparison of receiver-side key exposure under partial RU compromise.}
\label{tab:key-exposure}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{p{0.23\columnwidth} p{0.27\columnwidth} p{0.37\columnwidth}}
\toprule
\textbf{Scheme} & \textbf{RU-held future-forgery secret?} & \textbf{Impact of RU memory disclosure} \\ß
\midrule
Shared group MAC
& Yes, group-wide
& Future forgery for the entire RU group. \\
\addlinespace[1pt]

Pairwise symmetric MAC
& Yes, per association
& Future forgery for the compromised DU--RU association until rekeying. \\
\addlinespace[1pt]

Conventional TESLA
& No
& Reveals expired verification keys, but delayed verification disrupts real-time PTP. \\
\addlinespace[1pt]

\sys
& No
& Reveals expired verification state only; future keys remain hidden while samples are applied immediately and corrected if invalid. \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[htbp]
% \centering
% \caption{Comparison of TESLA-based Synchronization Schemes}
% \label{tab:tesla_comparison}
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \textbf{Scheme} & \textbf{Security Level} & \textbf{Loss Tolerance} & \textbf{Computation} & \textbf{Complexity} \\
% \hline
% S1 & Medium & Low & Low & Simple \\
% \hline
% S2 & Medium & High & Medium & Moderate \\
% \hline
% S3 & High & Low & High & Complex \\
% \hline
% S4 & Medium & Medium & Low & Moderate \\
% \hline
% \end{tabular}
% \end{table}


% \begin{table*}[htbp]
% \centering
% \caption{Detailed Comparison of TESLA-based Time Synchronization Schemes}
% \label{tab:tesla_detailed_comparison}
% \renewcommand{\arraystretch}{1.4}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|p{4cm}|c|c|c|c|}
% \hline
% \textbf{Aspect} & \textbf{Interval Key + Final Msg} & \textbf{Cycle Key + Aggregated Msgs} & \textbf{Round Key + Single Msg MACs} & \textbf{Round Key + Joint MAC in Delay\_Resp} \\
% \hline
% \textbf{Security Level} & Medium & Medium & High & Medium \\
% \hline
% \textbf{Loss Tolerance} & Low (last message critical) & High (statistical fusion) & Low (any loss breaks round) & Medium (Delay\_Resp critical) \\
% \hline
% \textbf{Bandwidth Overhead} & Low & Medium (more messages processed) & High (MAC per message) & Low (MAC only in Delay\_Resp) \\
% \hline
% \textbf{Computation Load} & Low & Medium (aggregation/filtering) & High (many MACs + key switching) & Low (single MAC validation) \\
% \hline
% \textbf{Implementation Complexity} & Simple & Moderate & Complex & Moderate \\
% \hline
% \textbf{Key Management Complexity} & Low (1 key per cycle) & Low (same) & High (1 key per round) & High (1 key per round) \\
% \hline
% \textbf{Synchronization Accuracy} & Medium (may jitter) & High (averaging improves stability) & High (per-round precision) & Medium (depends on Delay\_Resp timing) \\
% \hline
% \textbf{Multicast Suitability} & Good & Good & Poor (per-node keys) & Moderate (shared Delay\_Resp hard in multicast) \\
% \hline
% \textbf{Replay Protection} & Partial (per cycle) & Partial & Strong (per message) & Strong (round-bounded) \\
% \hline
% \textbf{Storage Requirement} & Low (store 1–2 messages + 1 key) & Medium (store multiple messages per cycle + 1 key) & High (store 4 messages, 4 MACs, 1 key per round) & Medium (store 4 messages + 1 MAC + 1 key) \\
% \hline
% \end{tabular}
% }
% \end{table*}



==> tables/dim_compare.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of design dimensions for synchronization protection.}
\label{tab:design-dimensions}
\begin{tabular}{@{}p{3.2cm}p{4cm}p{8cm}@{}}
\toprule
\textbf{Dimension} & \textbf{Representative Options} & \textbf{Characteristics and Trade-offs} \\ 
\midrule

\textbf{Key Disclosure Frequency} 
& \textit{Shared Key}, \textit{Per-Interval Keying}, \textit{Per-Round Keying} 
& Defines how often authentication keys are rotated and disclosed.  
Higher frequency (e.g., per-round) reduces exposure and improves isolation but increases computation and key-management overhead. \\

% \addlinespace[4pt]
\midrule

\textbf{Synchronization Computation} 
& \textit{Final-Only Synchronization}, \textit{Aggregated Synchronization} 
& Determines how PTP message pairs are used to estimate clock offset and delay.  
Final-only minimizes maintained state and latency but is sensitive to packet loss;  
aggregated synchronization improves robustness to jitter and tampering at the cost of higher processing complexity. \\

% \addlinespace[4pt]
\midrule

\textbf{Authentication Application Timing} 
& \textit{Verify-then-Apply}, \textit{Apply-then-Verify} 
& Specifies when synchronization updates are applied relative to key disclosure.  
Verify-then-Apply ensures that only authenticated data affect timing, introducing disclosure-delay latency;  
Apply-then-Verify enables immediate updates for real-time responsiveness, with a short speculative vulnerability window. \\

\bottomrule
\end{tabular}
\end{table*}


==> tables/metrics.tex <==
\begin{table*}[ht]
\centering
\caption{Evaluation metrics used to assess timing accuracy, robustness, and system efficiency.}
\label{tab:metrics}
% \renewcommand{\arraystretch}{1.05}
\begin{tabular}{p{3.5cm} p{5cm} p{7cm}}
\toprule
\textbf{Category} & \textbf{Metric} & \textbf{Description} \\
\midrule

\multirow{3}{*}{\textbf{Timing Accuracy}} 
& RMS offset (ns) &
Steady-state synchronization accuracy between O-DU and O-RU. \\
& Mean frequency correction (ppb) &
Average servo adjustment required to track the master clock. \\
& One-way delay (ns) &
Average measured path delay using PTP Delay Request–Response. \\

\midrule
\multirow{3}{*}{\textbf{Stability}} 
& Offset variability (ns) &
Standard deviation of RMS offset, quantifying timing oscillation.\\
& Frequency variability (ppb) &
Standard deviation of frequency correction, indicating servo stability.\\
& Delay variability (ns) &
Standard deviation of one-way delay, reflecting path jitter.\\

\midrule
\multirow{3}{*}{\textbf{Security Robustness}} 
& Attack-induced RMS offset (ns) &
Offset under varying MITM tampering rates $p$, measuring disruption resilience.\\
& Attack-induced frequency drift (ppb) &
Frequency correction under attack, showing servo disturbance.\\
& Attack-induced delay (ns) &
One-way delay under attack, capturing adversarial manipulation effects.\\

\midrule
\multirow{4}{*}{\textbf{System Overhead}} 
& CPU utilization (\%) &
User and kernel CPU load on O-DU and O-RU while processing PTP traffic.\\
& Memory footprint (MiB) &
Resident memory used by synchronization and authentication modules.\\
& PTP packet size (bytes) &
Per–message-type overhead contributed by authentication TLVs.\\
& Authentication cost (qualitative) &
Relative per-message/ per-round cryptographic work across schemes.\\

\midrule
\multirow{3}{*}{\textbf{\makecell[l]{Microarchitectural\\Efficiency}}}
& Instructions per cycle (IPC) &
Overall pipeline efficiency while running PTP + authentication logic.\\
& Stalled cycles (frontend/backend) &
Fraction of cycles stalled due to fetch, execution, or memory bottlenecks.\\
& Context switches (events/s) &
Scheduling and buffering overhead affecting timing determinism.\\

\bottomrule
\end{tabular}
\end{table*}


==> tables/protocol_symbols.tex <==
\begin{table*}[t]
\centering
\caption{\sys Parameters and State Variables.}
\label{tab:alg1-params-state}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\linewidth}{@{} l l X @{}}
\toprule
\textbf{Category} & \textbf{Name} & \textbf{Description} \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Parameters}} \\
\midrule
 & $d$ & Key disclosure delay (in rounds). \\
 & $r$ & Rounds per second (so $T_{\text{round}} = 1/r$). \\
 & $S_{\max}$ & Maximum slew (frequency offset bound). \\
 & $\tau_{\text{verify}}$ & Verification timeout ($\ge (d+\text{margin})\cdot T_{\text{round}}$). \\
 & $W_{\text{seq}}$ & Sequence forward-jump window (optional bound). \\
 & $R_{\text{roll}}$ & Rollover pre-announce margin ($\ge d+\text{loss margin}$). \\
 & $w,\,K_{\text{win}}$ & Window retransmission parameters ($w$ small, $K_{\text{win}}$ low rate). \\
\midrule
\multicolumn{3}{@{}l}{\textbf{DU State}} \\
\midrule
 & \texttt{epoch\_id}, \texttt{seq} & Current epoch identifier and round sequence number. \\
 & \texttt{key\_source(epoch\_id)} & Provides $K_{\text{seq}}$ (via precomputed array or checkpoints). \\
 & \texttt{discloseQ} & Queue of $(\texttt{seq}, K_{\texttt{seq}}, \texttt{disclose\_at\_seq}=\texttt{seq}+d)$. \\
 & \texttt{next\_commit\_pending?} & Tracks whether \texttt{NextCommit} for epoch+1 is pending (during rollover). \\
\midrule
\multicolumn{3}{@{}l}{\textbf{RU State}} \\
\midrule
 & \texttt{expected\_seq} & Next expected sequence number. \\
 & \texttt{measbuf[seq]} & Stored timestamps/messages needed to compute offset. \\
 & \texttt{macbuf[seq]} & MAC for \texttt{seq} (from Delay\_Resp / PrevMAC / WinMAC). \\
 & \texttt{ledger[seq]} & Applied control inputs for \texttt{seq} (for correction). \\
 & \texttt{verify\_deadline[seq]} & Per-round verification deadline for garbage collection. \\
 & \texttt{committed\_servo\_state} & Verified-only controller state (optional). \\
 & \texttt{speculative\_servo\_state} & Realtime controller state. \\
 & \texttt{Commit\_cur}, \texttt{Commit\_next}, \texttt{epoch\_id\_cur}, \texttt{switch\_seq} & Current/next commitment, current epoch id, and scheduled switch sequence. \\
\bottomrule
\end{tabularx}
\end{table*}


